Cutting Corners

We define and study a class of subshifts of finite type (SFTs) defined by a family of allowed patterns of the same shape where, for any contents of the shape minus a corner, the number of ways to fill in the corner is the same. The main results are that for such an SFT, a locally legal pattern of convex shape is globally legal, and there is a measure that samples uniformly on all convex sets. Under suitable computability assumptions, this measure can be sampled, and legal configurations counted and enumerated, effectively and efficiently. We show by example that these subshifts need not admit a group (more generally unital magma or quasigroup) structure by shift-commuting continuous operations. Our approach to convexity is axiomatic, and only requires an abstract convex geometry that is "midpointed with respect to the shape". We construct such convex geometries on several groups, in particular all strongly polycyclic groups and free groups. We also show some other methods for sampling finite patterns, one based on orderings and one based on contructing new "independent sets" from old. We also show a link to conjectures of Gottshalk and Kaplansky.

==> adicsfight3.tex <==
                               .a                                                                                         
                              ..aa                                                                                        
                             .. aba                                                                                       
                           ...  a  a                                                                                      
                          ..    aa aa                                                                                     
                        ...     abaaba                                                                                    
                       ..       a  b  a                                                                                   
                     ...        aa bb aa                                                                                  
                    ..          ababababa                                                                                 
                  ...           a        a                                                                                
                 ..             aa       aa                                                                               
               ...              aba      aba                                                                              
              ..                a  a     a  a                                                                             
             ..                 aa aa    aa aa                                                                            
           ...                  abaaba   abaaba                                                                           
          ..                    a  b  a  a  b  a                                                                          
        ...                     aa bb aa aa bb aa                                                                         
       ..                       ababababaababababa                                                                        
     ...                        a        b        a                                                                       
    ..                          aa       bb       aa                                                                      
  ...                           aba      bab      aba                                                                     
 ..                             a  a     b  b     a  a                                                                    
B.                              aa aa    bb bb    aa aa                                                                   
BB                              abaaba   babbab   abaaba                                                                  
B B                             a  b  a  b  a  b  a  b  a                                                                 
BBBB                            aa bb aa bb aa bb aa bb aa                                                                
B   B                           abababababababababababababa                                                               
BB  BB                          a                          a                                                              
B B B B                         aa                         aa                                                             
BBBBBBBB                        aba                        aba                                                            
B       B                       a  a                       a  a                                                           
BB      BB                      aa aa                      aa aa                                                          
B B     B B                     abaaba                     abaaba                                                         
BBBB    BBBB                    a  b  a                    a  b  a                                                        
B   B   B   B                   aa bb aa                   aa bb aa                                                       
BB  BB  BB  BB                  ababababa                  ababababa                                                      
B B B B B B B B                 a        a                 a        a                                                     
BBBBBBBBBBBBBBBB                aa       aa                aa       aa                                                    
B               B               aba      aba               aba      aba                                                   
BB              BB              a  a     a  a              a  a     a  a                                                  
B B             B B             aa aa    aa aa             aa aa    aa aa                                                 
BBBB            BBBB            abaaba   abaaba            abaaba   abaaba                                                
B   B           B   B           a  b  a  a  b  a           a  b  a  a  b  a                                               
BB  BB          BB  BB          aa bb aa aa bb aa          aa bb aa aa bb aa                                              
B B B B         B B B B         ababababaababababa         ababababaababababa                                             
BBBBBBBB        BBBBBBBB        a        b        a        a        b        a                                            
B       B       B       B       aa       bb       aa       aa       bb       aa                                           
BB      BB      BB      BB      aba      bab      aba      aba      bab      aba                                          
B B     B B     B B     B B     a  a     b  b     a  a     a  a     b  b     a  a                                         
BBBB    BBBB    BBBB    BBBB    aa aa    bb bb    aa aa    aa aa    bb bb    aa aa                                        
B   B   B   B   B   B   B   B   abaaba   babbab   abaaba   abaaba   babbab   abaaba                                       
BB  BB  BB  BB  BB  BB  BB  BB  a  b  a  b  a  b  a  b  a  a  b  a  b  a  b  a  b  a                                      
B B B B B B B B B B B B B B B B aa bb aa bb aa bb aa bb aa aa bb aa bb aa bb aa bb aa                                     
BBBBBBBBBBBBBBBBBBBBBBBBBBBBBBBBabababababababababababababaabababababababababababababa                                    
B                               *                          b                          a                                   
BB                              **                         bb                         aa                                  
B B                             * *                        bab                        aba                                 
BBBB                            ****                       b  b                       a  a                                
B   B                           *   *                      bb bb                      aa aa                               
BB  BB                          **  **                     babbab                     abaaba                              
B B B B                         * * * *                    b  a  b                    a  b  a                             
BBBBBBBB                        ********                   bb aa bb                   aa bb aa                            
B       B                       *       *                  babababab                  ababababa                           
BB      BB                      **      **                 b        b                 a        a                          
B B     B B                     * *     * *                bb       bb                aa       aa                         
BBBB    BBBB                    ****    ****               bab      bab               aba      aba                        
B   B   B   B                   *   *   *   *              b  b     b  b              a  a     a  a                       
BB  BB  BB  BB                  **  **  **  **             bb bb    bb bb             aa aa    aa aa                      
B B B B B B B B                 * * * * * * * *            babbab   babbab            abaaba   abaaba                     
BBBBBBBBBBBBBBBB                ****************           b  a  b  b  a  b           a  b  a  a  b  a                    
B               B               *               *          bb aa bb bb aa bb          aa bb aa aa bb aa                   
BB              BB              **              **         bababababbabababab         ababababaababababa                  
B B             B B             * *             * *        b        a        b        a        b        a                 
BBBB            BBBB            ****            ****       bb       aa       bb       aa       bb       aa                
B   B           B   B           *   *           *   *      bab      aba      bab      aba      bab      aba               
BB  BB          BB  BB          **  **          **  **     b  b     a  a     b  b     a  a     b  b     a  a              
B B B B         B B B B         * * * *         * * * *    bb bb    aa aa    bb bb    aa aa    bb bb    aa aa             
BBBBBBBB        BBBBBBBB        ********        ********   babbab   abaaba   babbab   abaaba   babbab   abaaba            
B       B       B       B       *       *       *       *  b  a  b  a  b  a  b  a  b  a  b  a  b  a  b  a  b  a           
BB      BB      BB      BB      **      **      **      ** bb aa bb aa bb aa bb aa bb aa bb aa bb aa bb aa bb aa          
B B     B B     B B     B B     * *     * *     * *     * *bababababababababababababababababababababababababababa         
BBBB    BBBB    BBBB    BBBB    ****    ****    ****    ***B                                                     a        
B   B   B   B   B   B   B   B   *   *   *   *   *   *   *  bB                                                    aa       
BB  BB  BB  BB  BB  BB  BB  BB  **  **  **  **  **  **  ** b*B                                                   aba      
B B B B B B B B B B B B B B B B * * * * * * * * * * * * * *bAbB                                                  a  a     
BBBBBBBBBBBBBBBBBBBBBBBBBBBBBBBB***************************BB**B                                                 aa aa    
B                               a                          b a bB                                                abaaba   
BB                              aa                         bbaab*B                                               a  b  a  
B B                             aba                        ba b AbB                                              aa bb aa 
BBBB                            a  a                       b abbA**B                                             ababababa

==> tree_convex_ordering2.tex <==
\draw (0, 0) -- (3, 0);
\draw (3, 0) -- (4.5, 0.0);
\draw (4.5, 0.0) -- (5.25, 0.0);
\draw (5.25, 0.0) -- (5.625, 0.0);
\draw (5.25, 0.0) -- (5.25, 0.375);
\draw (5.25, 0.0) -- (5.25, -0.375);
\draw (4.5, 0.0) -- (4.5, 0.75);
\draw (4.5, 0.75) -- (4.875, 0.75);
\draw (4.5, 0.75) -- (4.125, 0.75);
\draw (4.5, 0.75) -- (4.5, 1.125);
\draw (4.5, 0.0) -- (4.5, -0.75);
\draw (4.5, -0.75) -- (4.875, -0.75);
\draw (4.5, -0.75) -- (4.125, -0.75);
\draw (4.5, -0.75) -- (4.5, -1.125);
\draw (3, 0) -- (3.0, 1.5);
\draw (3.0, 1.5) -- (3.75, 1.5);
\draw (3.75, 1.5) -- (4.125, 1.5);
\draw (3.75, 1.5) -- (3.75, 1.875);
\draw (3.75, 1.5) -- (3.75, 1.125);
\draw (3.0, 1.5) -- (2.25, 1.5);
\draw (2.25, 1.5) -- (1.875, 1.5);
\draw (2.25, 1.5) -- (2.25, 1.875);
\draw (2.25, 1.5) -- (2.25, 1.125);
\draw (3.0, 1.5) -- (3.0, 2.25);
\draw (3.0, 2.25) -- (3.375, 2.25);
\draw (3.0, 2.25) -- (2.625, 2.25);
\draw (3.0, 2.25) -- (3.0, 2.625);
\draw (3, 0) -- (3.0, -1.5);
\draw (3.0, -1.5) -- (3.75, -1.5);
\draw (3.75, -1.5) -- (4.125, -1.5);
\draw (3.75, -1.5) -- (3.75, -1.125);
\draw (3.75, -1.5) -- (3.75, -1.875);
\draw (3.0, -1.5) -- (2.25, -1.5);
\draw (2.25, -1.5) -- (1.875, -1.5);
\draw (2.25, -1.5) -- (2.25, -1.125);
\draw (2.25, -1.5) -- (2.25, -1.875);
\draw (3.0, -1.5) -- (3.0, -2.25);
\draw (3.0, -2.25) -- (3.375, -2.25);
\draw (3.0, -2.25) -- (2.625, -2.25);
\draw (3.0, -2.25) -- (3.0, -2.625);
\draw (0, 0) -- (-3, 0);
\draw (-3, 0) -- (-4.5, 0.0);
\draw (-4.5, 0.0) -- (-5.25, 0.0);
\draw (-5.25, 0.0) -- (-5.625, 0.0);
\draw (-5.25, 0.0) -- (-5.25, 0.375);
\draw (-5.25, 0.0) -- (-5.25, -0.375);
\draw (-4.5, 0.0) -- (-4.5, 0.75);
\draw (-4.5, 0.75) -- (-4.125, 0.75);
\draw (-4.5, 0.75) -- (-4.875, 0.75);
\draw (-4.5, 0.75) -- (-4.5, 1.125);
\draw (-4.5, 0.0) -- (-4.5, -0.75);
\draw (-4.5, -0.75) -- (-4.125, -0.75);
\draw (-4.5, -0.75) -- (-4.875, -0.75);
\draw (-4.5, -0.75) -- (-4.5, -1.125);
\draw (-3, 0) -- (-3.0, 1.5);
\draw (-3.0, 1.5) -- (-2.25, 1.5);
\draw (-2.25, 1.5) -- (-1.875, 1.5);
\draw (-2.25, 1.5) -- (-2.25, 1.875);
\draw (-2.25, 1.5) -- (-2.25, 1.125);
\draw (-3.0, 1.5) -- (-3.75, 1.5);
\draw (-3.75, 1.5) -- (-4.125, 1.5);
\draw (-3.75, 1.5) -- (-3.75, 1.875);
\draw (-3.75, 1.5) -- (-3.75, 1.125);
\draw (-3.0, 1.5) -- (-3.0, 2.25);
\draw (-3.0, 2.25) -- (-2.625, 2.25);
\draw (-3.0, 2.25) -- (-3.375, 2.25);
\draw (-3.0, 2.25) -- (-3.0, 2.625);
\draw (-3, 0) -- (-3.0, -1.5);
\draw (-3.0, -1.5) -- (-2.25, -1.5);
\draw (-2.25, -1.5) -- (-1.875, -1.5);
\draw (-2.25, -1.5) -- (-2.25, -1.125);
\draw (-2.25, -1.5) -- (-2.25, -1.875);
\draw (-3.0, -1.5) -- (-3.75, -1.5);
\draw (-3.75, -1.5) -- (-4.125, -1.5);
\draw (-3.75, -1.5) -- (-3.75, -1.125);
\draw (-3.75, -1.5) -- (-3.75, -1.875);
\draw (-3.0, -1.5) -- (-3.0, -2.25);
\draw (-3.0, -2.25) -- (-2.625, -2.25);
\draw (-3.0, -2.25) -- (-3.375, -2.25);
\draw (-3.0, -2.25) -- (-3.0, -2.625);
\draw (0, 0) -- (0, 3);
\draw (0, 3) -- (1.5, 3.0);
\draw (1.5, 3.0) -- (2.25, 3.0);
\draw (2.25, 3.0) -- (2.625, 3.0);
\draw (2.25, 3.0) -- (2.25, 3.375);
\draw (2.25, 3.0) -- (2.25, 2.625);
\draw (1.5, 3.0) -- (1.5, 3.75);
\draw (1.5, 3.75) -- (1.875, 3.75);
\draw (1.5, 3.75) -- (1.125, 3.75);
\draw (1.5, 3.75) -- (1.5, 4.125);
\draw (1.5, 3.0) -- (1.5, 2.25);
\draw (1.5, 2.25) -- (1.875, 2.25);
\draw (1.5, 2.25) -- (1.125, 2.25);
\draw (1.5, 2.25) -- (1.5, 1.875);
\draw (0, 3) -- (-1.5, 3.0);
\draw (-1.5, 3.0) -- (-2.25, 3.0);
\draw (-2.25, 3.0) -- (-2.625, 3.0);
\draw (-2.25, 3.0) -- (-2.25, 3.375);
\draw (-2.25, 3.0) -- (-2.25, 2.625);
\draw (-1.5, 3.0) -- (-1.5, 3.75);
\draw (-1.5, 3.75) -- (-1.125, 3.75);
\draw (-1.5, 3.75) -- (-1.875, 3.75);
\draw (-1.5, 3.75) -- (-1.5, 4.125);
\draw (-1.5, 3.0) -- (-1.5, 2.25);
\draw (-1.5, 2.25) -- (-1.125, 2.25);
\draw (-1.5, 2.25) -- (-1.875, 2.25);
\draw (-1.5, 2.25) -- (-1.5, 1.875);
\draw (0, 3) -- (0.0, 4.5);
\draw (0.0, 4.5) -- (0.75, 4.5);
\draw (0.75, 4.5) -- (1.125, 4.5);
\draw (0.75, 4.5) -- (0.75, 4.875);
\draw (0.75, 4.5) -- (0.75, 4.125);
\draw (0.0, 4.5) -- (-0.75, 4.5);
\draw (-0.75, 4.5) -- (-1.125, 4.5);
\draw (-0.75, 4.5) -- (-0.75, 4.875);
\draw (-0.75, 4.5) -- (-0.75, 4.125);
\draw (0.0, 4.5) -- (0.0, 5.25);
\draw (0.0, 5.25) -- (0.375, 5.25);
\draw (0.0, 5.25) -- (-0.375, 5.25);
\draw (0.0, 5.25) -- (0.0, 5.625);
\draw (0, 0) -- (0, -3);
\draw (0, -3) -- (1.5, -3.0);
\draw (1.5, -3.0) -- (2.25, -3.0);
\draw (2.25, -3.0) -- (2.625, -3.0);
\draw (2.25, -3.0) -- (2.25, -2.625);
\draw (2.25, -3.0) -- (2.25, -3.375);
\draw (1.5, -3.0) -- (1.5, -2.25);
\draw (1.5, -2.25) -- (1.875, -2.25);
\draw (1.5, -2.25) -- (1.125, -2.25);
\draw (1.5, -2.25) -- (1.5, -1.875);
\draw (1.5, -3.0) -- (1.5, -3.75);
\draw (1.5, -3.75) -- (1.875, -3.75);
\draw (1.5, -3.75) -- (1.125, -3.75);
\draw (1.5, -3.75) -- (1.5, -4.125);
\draw (0, -3) -- (-1.5, -3.0);
\draw (-1.5, -3.0) -- (-2.25, -3.0);
\draw (-2.25, -3.0) -- (-2.625, -3.0);
\draw (-2.25, -3.0) -- (-2.25, -2.625);
\draw (-2.25, -3.0) -- (-2.25, -3.375);
\draw (-1.5, -3.0) -- (-1.5, -2.25);
\draw (-1.5, -2.25) -- (-1.125, -2.25);
\draw (-1.5, -2.25) -- (-1.875, -2.25);
\draw (-1.5, -2.25) -- (-1.5, -1.875);
\draw (-1.5, -3.0) -- (-1.5, -3.75);
\draw (-1.5, -3.75) -- (-1.125, -3.75);
\draw (-1.5, -3.75) -- (-1.875, -3.75);
\draw (-1.5, -3.75) -- (-1.5, -4.125);
\draw (0, -3) -- (0.0, -4.5);
\draw (0.0, -4.5) -- (0.75, -4.5);
\draw (0.75, -4.5) -- (1.125, -4.5);
\draw (0.75, -4.5) -- (0.75, -4.125);
\draw (0.75, -4.5) -- (0.75, -4.875);
\draw (0.0, -4.5) -- (-0.75, -4.5);
\draw (-0.75, -4.5) -- (-1.125, -4.5);
\draw (-0.75, -4.5) -- (-0.75, -4.125);
\draw (-0.75, -4.5) -- (-0.75, -4.875);
\draw (0.0, -4.5) -- (0.0, -5.25);
\draw (0.0, -5.25) -- (0.375, -5.25);
\draw (0.0, -5.25) -- (-0.375, -5.25);
\draw (0.0, -5.25) -- (0.0, -5.625);
\node[draw,circle,fill=white,inner sep=0,minimum size=4mm] () at (0,0) {\tiny{13}};
\node[draw,circle,fill=black!5.0!white,inner sep=0,minimum size=4mm] () at (3,0) {\tiny{21}};
\node[draw,circle,fill=black!7.75!white,inner sep=0,minimum size=4mm] () at (4.5,0.0) {\tiny{32}};
\node[draw,circle,fill=black!16.25!white,inner sep=0,minimum size=4mm] () at (5.25,0.0) {\tiny{66}};
\node[draw,circle,fill=black!38.75!white,inner sep=0,minimum size=4mm] () at (5.625,0.0) {\tiny{156}};
\node[draw,circle,fill=black!23.25!white,inner sep=0,minimum size=4mm] () at (5.25,0.375) {\tiny{94}};
\node[draw,circle,fill=black!26.5!white,inner sep=0,minimum size=4mm] () at (5.25,-0.375) {\tiny{107}};
\node[draw,circle,fill=black!19.25!white,inner sep=0,minimum size=4mm] () at (4.5,0.75) {\tiny{78}};
\node[draw,circle,fill=black!26.0!white,inner sep=0,minimum size=4mm] () at (4.875,0.75) {\tiny{105}};
\node[draw,circle,fill=black!24.0!white,inner sep=0,minimum size=4mm] () at (4.125,0.75) {\tiny{97}};
\node[draw,circle,fill=black!36.0!white,inner sep=0,minimum size=4mm] () at (4.5,1.125) {\tiny{145}};
\node[draw,circle,fill=black!16.5!white,inner sep=0,minimum size=4mm] () at (4.5,-0.75) {\tiny{67}};
\node[draw,circle,fill=black!34.5!white,inner sep=0,minimum size=4mm] () at (4.875,-0.75) {\tiny{139}};
\node[draw,circle,fill=black!31.5!white,inner sep=0,minimum size=4mm] () at (4.125,-0.75) {\tiny{127}};
\node[draw,circle,fill=black!21.25!white,inner sep=0,minimum size=4mm] () at (4.5,-1.125) {\tiny{86}};
\node[draw,circle,fill=black!11.0!white,inner sep=0,minimum size=4mm] () at (3.0,1.5) {\tiny{45}};
\node[draw,circle,fill=black!15.75!white,inner sep=0,minimum size=4mm] () at (3.75,1.5) {\tiny{64}};
\node[draw,circle,fill=black!28.25!white,inner sep=0,minimum size=4mm] () at (4.125,1.5) {\tiny{114}};
\node[draw,circle,fill=black!26.25!white,inner sep=0,minimum size=4mm] () at (3.75,1.875) {\tiny{106}};
\node[draw,circle,fill=black!38.0!white,inner sep=0,minimum size=4mm] () at (3.75,1.125) {\tiny{153}};
\node[draw,circle,fill=black!14.5!white,inner sep=0,minimum size=4mm] () at (2.25,1.5) {\tiny{59}};
\node[draw,circle,fill=black!33.75!white,inner sep=0,minimum size=4mm] () at (1.875,1.5) {\tiny{136}};
\node[draw,circle,fill=black!39.25!white,inner sep=0,minimum size=4mm] () at (2.25,1.875) {\tiny{158}};
\node[draw,circle,fill=black!21.0!white,inner sep=0,minimum size=4mm] () at (2.25,1.125) {\tiny{85}};
\node[draw,circle,fill=black!16.75!white,inner sep=0,minimum size=4mm] () at (3.0,2.25) {\tiny{68}};
\node[draw,circle,fill=black!31.25!white,inner sep=0,minimum size=4mm] () at (3.375,2.25) {\tiny{126}};
\node[draw,circle,fill=black!30.5!white,inner sep=0,minimum size=4mm] () at (2.625,2.25) {\tiny{123}};
\node[draw,circle,fill=black!28.5!white,inner sep=0,minimum size=4mm] () at (3.0,2.625) {\tiny{115}};
\node[draw,circle,fill=black!8.25!white,inner sep=0,minimum size=4mm] () at (3.0,-1.5) {\tiny{34}};
\node[draw,circle,fill=black!13.25!white,inner sep=0,minimum size=4mm] () at (3.75,-1.5) {\tiny{54}};
\node[draw,circle,fill=black!27.75!white,inner sep=0,minimum size=4mm] () at (4.125,-1.5) {\tiny{112}};
\node[draw,circle,fill=black!22.5!white,inner sep=0,minimum size=4mm] () at (3.75,-1.125) {\tiny{91}};
\node[draw,circle,fill=black!33.5!white,inner sep=0,minimum size=4mm] () at (3.75,-1.875) {\tiny{135}};
\node[draw,circle,fill=black!13.0!white,inner sep=0,minimum size=4mm] () at (2.25,-1.5) {\tiny{53}};
\node[draw,circle,fill=black!26.75!white,inner sep=0,minimum size=4mm] () at (1.875,-1.5) {\tiny{108}};
\node[draw,circle,fill=black!34.25!white,inner sep=0,minimum size=4mm] () at (2.25,-1.125) {\tiny{138}};
\node[draw,circle,fill=black!30.25!white,inner sep=0,minimum size=4mm] () at (2.25,-1.875) {\tiny{122}};
\node[draw,circle,fill=black!14.75!white,inner sep=0,minimum size=4mm] () at (3.0,-2.25) {\tiny{60}};
\node[draw,circle,fill=black!31.75!white,inner sep=0,minimum size=4mm] () at (3.375,-2.25) {\tiny{128}};
\node[draw,circle,fill=black!37.0!white,inner sep=0,minimum size=4mm] () at (2.625,-2.25) {\tiny{149}};
\node[draw,circle,fill=black!20.5!white,inner sep=0,minimum size=4mm] () at (3.0,-2.625) {\tiny{83}};
\node[draw,circle,fill=black!5.25!white,inner sep=0,minimum size=4mm] () at (-3,0) {\tiny{22}};
\node[draw,circle,fill=black!8.0!white,inner sep=0,minimum size=4mm] () at (-4.5,0.0) {\tiny{33}};
\node[draw,circle,fill=black!14.0!white,inner sep=0,minimum size=4mm] () at (-5.25,0.0) {\tiny{57}};
\node[draw,circle,fill=black!25.25!white,inner sep=0,minimum size=4mm] () at (-5.625,0.0) {\tiny{102}};
\node[draw,circle,fill=black!36.25!white,inner sep=0,minimum size=4mm] () at (-5.25,0.375) {\tiny{146}};
\node[draw,circle,fill=black!21.5!white,inner sep=0,minimum size=4mm] () at (-5.25,-0.375) {\tiny{87}};
\node[draw,circle,fill=black!17.25!white,inner sep=0,minimum size=4mm] () at (-4.5,0.75) {\tiny{70}};
\node[draw,circle,fill=black!36.5!white,inner sep=0,minimum size=4mm] () at (-4.125,0.75) {\tiny{147}};
\node[draw,circle,fill=black!34.75!white,inner sep=0,minimum size=4mm] () at (-4.875,0.75) {\tiny{140}};
\node[draw,circle,fill=black!29.75!white,inner sep=0,minimum size=4mm] () at (-4.5,1.125) {\tiny{120}};
\node[draw,circle,fill=black!13.75!white,inner sep=0,minimum size=4mm] () at (-4.5,-0.75) {\tiny{56}};
\node[draw,circle,fill=black!22.75!white,inner sep=0,minimum size=4mm] () at (-4.125,-0.75) {\tiny{92}};
\node[draw,circle,fill=black!27.0!white,inner sep=0,minimum size=4mm] () at (-4.875,-0.75) {\tiny{109}};
\node[draw,circle,fill=black!24.25!white,inner sep=0,minimum size=4mm] () at (-4.5,-1.125) {\tiny{98}};
\node[draw,circle,fill=black!10.25!white,inner sep=0,minimum size=4mm] () at (-3.0,1.5) {\tiny{42}};
\node[draw,circle,fill=black!15.25!white,inner sep=0,minimum size=4mm] () at (-2.25,1.5) {\tiny{62}};
\node[draw,circle,fill=black!20.0!white,inner sep=0,minimum size=4mm] () at (-1.875,1.5) {\tiny{81}};
\node[draw,circle,fill=black!37.25!white,inner sep=0,minimum size=4mm] () at (-2.25,1.875) {\tiny{150}};
\node[draw,circle,fill=black!28.75!white,inner sep=0,minimum size=4mm] () at (-2.25,1.125) {\tiny{116}};
\node[draw,circle,fill=black!18.5!white,inner sep=0,minimum size=4mm] () at (-3.75,1.5) {\tiny{75}};
\node[draw,circle,fill=black!35.25!white,inner sep=0,minimum size=4mm] () at (-4.125,1.5) {\tiny{142}};
\node[draw,circle,fill=black!20.75!white,inner sep=0,minimum size=4mm] () at (-3.75,1.875) {\tiny{84}};
\node[draw,circle,fill=black!33.0!white,inner sep=0,minimum size=4mm] () at (-3.75,1.125) {\tiny{133}};
\node[draw,circle,fill=black!19.0!white,inner sep=0,minimum size=4mm] () at (-3.0,2.25) {\tiny{77}};
\node[draw,circle,fill=black!32.0!white,inner sep=0,minimum size=4mm] () at (-2.625,2.25) {\tiny{129}};
\node[draw,circle,fill=black!32.5!white,inner sep=0,minimum size=4mm] () at (-3.375,2.25) {\tiny{131}};
\node[draw,circle,fill=black!34.0!white,inner sep=0,minimum size=4mm] () at (-3.0,2.625) {\tiny{137}};
\node[draw,circle,fill=black!9.75!white,inner sep=0,minimum size=4mm] () at (-3.0,-1.5) {\tiny{40}};
\node[draw,circle,fill=black!17.75!white,inner sep=0,minimum size=4mm] () at (-2.25,-1.5) {\tiny{72}};
\node[draw,circle,fill=black!37.75!white,inner sep=0,minimum size=4mm] () at (-1.875,-1.5) {\tiny{152}};
\node[draw,circle,fill=black!27.25!white,inner sep=0,minimum size=4mm] () at (-2.25,-1.125) {\tiny{110}};
\node[draw,circle,fill=black!35.0!white,inner sep=0,minimum size=4mm] () at (-2.25,-1.875) {\tiny{141}};
\node[draw,circle,fill=black!18.75!white,inner sep=0,minimum size=4mm] () at (-3.75,-1.5) {\tiny{76}};
\node[draw,circle,fill=black!23.0!white,inner sep=0,minimum size=4mm] () at (-4.125,-1.5) {\tiny{93}};
\node[draw,circle,fill=black!29.5!white,inner sep=0,minimum size=4mm] () at (-3.75,-1.125) {\tiny{119}};
\node[draw,circle,fill=black!27.5!white,inner sep=0,minimum size=4mm] () at (-3.75,-1.875) {\tiny{111}};
\node[draw,circle,fill=black!19.75!white,inner sep=0,minimum size=4mm] () at (-3.0,-2.25) {\tiny{80}};
\node[draw,circle,fill=black!24.75!white,inner sep=0,minimum size=4mm] () at (-2.625,-2.25) {\tiny{100}};
\node[draw,circle,fill=black!30.0!white,inner sep=0,minimum size=4mm] () at (-3.375,-2.25) {\tiny{121}};
\node[draw,circle,fill=black!24.5!white,inner sep=0,minimum size=4mm] () at (-3.0,-2.625) {\tiny{99}};
\node[draw,circle,fill=black!3.5!white,inner sep=0,minimum size=4mm] () at (0,3) {\tiny{15}};
\node[draw,circle,fill=black!11.25!white,inner sep=0,minimum size=4mm] () at (1.5,3.0) {\tiny{46}};
\node[draw,circle,fill=black!13.5!white,inner sep=0,minimum size=4mm] () at (2.25,3.0) {\tiny{55}};
\node[draw,circle,fill=black!38.25!white,inner sep=0,minimum size=4mm] () at (2.625,3.0) {\tiny{154}};
\node[draw,circle,fill=black!29.0!white,inner sep=0,minimum size=4mm] () at (2.25,3.375) {\tiny{117}};
\node[draw,circle,fill=black!35.5!white,inner sep=0,minimum size=4mm] () at (2.25,2.625) {\tiny{143}};
\node[draw,circle,fill=black!17.5!white,inner sep=0,minimum size=4mm] () at (1.5,3.75) {\tiny{71}};
\node[draw,circle,fill=black!37.5!white,inner sep=0,minimum size=4mm] () at (1.875,3.75) {\tiny{151}};
\node[draw,circle,fill=black!40.0!white,inner sep=0,minimum size=4mm] () at (1.125,3.75) {\tiny{161}};
\node[draw,circle,fill=black!38.5!white,inner sep=0,minimum size=4mm] () at (1.5,4.125) {\tiny{155}};
\node[draw,circle,fill=black!12.75!white,inner sep=0,minimum size=4mm] () at (1.5,2.25) {\tiny{52}};
\node[draw,circle,fill=black!31.0!white,inner sep=0,minimum size=4mm] () at (1.875,2.25) {\tiny{125}};
\node[draw,circle,fill=black!25.5!white,inner sep=0,minimum size=4mm] () at (1.125,2.25) {\tiny{103}};
\node[draw,circle,fill=black!22.25!white,inner sep=0,minimum size=4mm] () at (1.5,1.875) {\tiny{90}};
\node[draw,circle,fill=black!12.25!white,inner sep=0,minimum size=4mm] () at (-1.5,3.0) {\tiny{50}};
\node[draw,circle,fill=black!15.0!white,inner sep=0,minimum size=4mm] () at (-2.25,3.0) {\tiny{61}};
\node[draw,circle,fill=black!32.25!white,inner sep=0,minimum size=4mm] () at (-2.625,3.0) {\tiny{130}};
\node[draw,circle,fill=black!25.75!white,inner sep=0,minimum size=4mm] () at (-2.25,3.375) {\tiny{104}};
\node[draw,circle,fill=black!29.25!white,inner sep=0,minimum size=4mm] () at (-2.25,2.625) {\tiny{118}};
\node[draw,circle,fill=black!18.25!white,inner sep=0,minimum size=4mm] () at (-1.5,3.75) {\tiny{74}};
\node[draw,circle,fill=black!33.25!white,inner sep=0,minimum size=4mm] () at (-1.125,3.75) {\tiny{134}};
\node[draw,circle,fill=black!20.25!white,inner sep=0,minimum size=4mm] () at (-1.875,3.75) {\tiny{82}};
\node[draw,circle,fill=black!22.0!white,inner sep=0,minimum size=4mm] () at (-1.5,4.125) {\tiny{89}};
\node[draw,circle,fill=black!16.0!white,inner sep=0,minimum size=4mm] () at (-1.5,2.25) {\tiny{65}};
\node[draw,circle,fill=black!21.75!white,inner sep=0,minimum size=4mm] () at (-1.125,2.25) {\tiny{88}};
\node[draw,circle,fill=black!30.75!white,inner sep=0,minimum size=4mm] () at (-1.875,2.25) {\tiny{124}};
\node[draw,circle,fill=black!23.75!white,inner sep=0,minimum size=4mm] () at (-1.5,1.875) {\tiny{96}};
\node[draw,circle,fill=black!7.5!white,inner sep=0,minimum size=4mm] () at (0.0,4.5) {\tiny{31}};
\node[draw,circle,fill=black!18.0!white,inner sep=0,minimum size=4mm] () at (0.75,4.5) {\tiny{73}};
\node[draw,circle,fill=black!39.0!white,inner sep=0,minimum size=4mm] () at (1.125,4.5) {\tiny{157}};
\node[draw,circle,fill=black!39.75!white,inner sep=0,minimum size=4mm] () at (0.75,4.875) {\tiny{160}};
\node[draw,circle,fill=black!32.75!white,inner sep=0,minimum size=4mm] () at (0.75,4.125) {\tiny{132}};
\node[draw,circle,fill=black!12.5!white,inner sep=0,minimum size=4mm] () at (-0.75,4.5) {\tiny{51}};
\node[draw,circle,fill=black!25.0!white,inner sep=0,minimum size=4mm] () at (-1.125,4.5) {\tiny{101}};
\node[draw,circle,fill=black!23.5!white,inner sep=0,minimum size=4mm] () at (-0.75,4.875) {\tiny{95}};
\node[draw,circle,fill=black!36.75!white,inner sep=0,minimum size=4mm] () at (-0.75,4.125) {\tiny{148}};
\node[draw,circle,fill=black!15.5!white,inner sep=0,minimum size=4mm] () at (0.0,5.25) {\tiny{63}};
\node[draw,circle,fill=black!35.75!white,inner sep=0,minimum size=4mm] () at (0.375,5.25) {\tiny{144}};
\node[draw,circle,fill=black!39.5!white,inner sep=0,minimum size=4mm] () at (-0.375,5.25) {\tiny{159}};
\node[draw,circle,fill=black!28.0!white,inner sep=0,minimum size=4mm] () at (0.0,5.625) {\tiny{113}};
\node[draw,circle,fill=black!0.75!white,inner sep=0,minimum size=4mm] () at (0,-3) {\tiny{4}};
\node[draw,circle,fill=black!2.75!white,inner sep=0,minimum size=4mm] () at (1.5,-3.0) {\tiny{12}};
\node[draw,circle,fill=black!3.75!white,inner sep=0,minimum size=4mm] () at (2.25,-3.0) {\tiny{16}};
\node[draw,circle,fill=black!10.0!white,inner sep=0,minimum size=4mm] () at (2.625,-3.0) {\tiny{41}};
\node[draw,circle,fill=black!7.25!white,inner sep=0,minimum size=4mm] () at (2.25,-2.625) {\tiny{30}};
\node[draw,circle,fill=black!9.25!white,inner sep=0,minimum size=4mm] () at (2.25,-3.375) {\tiny{38}};
\node[draw,circle,fill=black!6.0!white,inner sep=0,minimum size=4mm] () at (1.5,-2.25) {\tiny{25}};
\node[draw,circle,fill=black!8.5!white,inner sep=0,minimum size=4mm] () at (1.875,-2.25) {\tiny{35}};
\node[draw,circle,fill=black!8.75!white,inner sep=0,minimum size=4mm] () at (1.125,-2.25) {\tiny{36}};
\node[draw,circle,fill=black!14.25!white,inner sep=0,minimum size=4mm] () at (1.5,-1.875) {\tiny{58}};
\node[draw,circle,fill=black!4.0!white,inner sep=0,minimum size=4mm] () at (1.5,-3.75) {\tiny{17}};
\node[draw,circle,fill=black!6.75!white,inner sep=0,minimum size=4mm] () at (1.875,-3.75) {\tiny{28}};
\node[draw,circle,fill=black!7.0!white,inner sep=0,minimum size=4mm] () at (1.125,-3.75) {\tiny{29}};
\node[draw,circle,fill=black!9.0!white,inner sep=0,minimum size=4mm] () at (1.5,-4.125) {\tiny{37}};
\node[draw,circle,fill=black!0.25!white,inner sep=0,minimum size=4mm] () at (-1.5,-3.0) {\tiny{2}};
\node[draw,circle,fill=black!0.5!white,inner sep=0,minimum size=4mm] () at (-2.25,-3.0) {\tiny{3}};
\node[draw,circle,fill=black!2.0!white,inner sep=0,minimum size=4mm] () at (-2.625,-3.0) {\tiny{9}};
\node[draw,circle,fill=black!5.5!white,inner sep=0,minimum size=4mm] () at (-2.25,-2.625) {\tiny{23}};
\node[draw,circle,fill=black!3.25!white,inner sep=0,minimum size=4mm] () at (-2.25,-3.375) {\tiny{14}};
\node[draw,circle,fill=black!0.0!white,inner sep=0,minimum size=4mm] () at (-1.5,-2.25) {\tiny{1}};
\node[draw,circle,fill=black!1.25!white,inner sep=0,minimum size=4mm] () at (-1.125,-2.25) {\tiny{6}};
\node[draw,circle,fill=black!1.5!white,inner sep=0,minimum size=4mm] () at (-1.875,-2.25) {\tiny{7}};
\node[draw,circle,fill=black!1.0!white,inner sep=0,minimum size=4mm] () at (-1.5,-1.875) {\tiny{5}};
\node[draw,circle,fill=black!1.75!white,inner sep=0,minimum size=4mm] () at (-1.5,-3.75) {\tiny{8}};
\node[draw,circle,fill=black!2.25!white,inner sep=0,minimum size=4mm] () at (-1.125,-3.75) {\tiny{10}};
\node[draw,circle,fill=black!4.25!white,inner sep=0,minimum size=4mm] () at (-1.875,-3.75) {\tiny{18}};
\node[draw,circle,fill=black!5.75!white,inner sep=0,minimum size=4mm] () at (-1.5,-4.125) {\tiny{24}};
\node[draw,circle,fill=black!2.5!white,inner sep=0,minimum size=4mm] () at (0.0,-4.5) {\tiny{11}};
\node[draw,circle,fill=black!4.75!white,inner sep=0,minimum size=4mm] () at (0.75,-4.5) {\tiny{20}};
\node[draw,circle,fill=black!6.5!white,inner sep=0,minimum size=4mm] () at (1.125,-4.5) {\tiny{27}};
\node[draw,circle,fill=black!10.5!white,inner sep=0,minimum size=4mm] () at (0.75,-4.125) {\tiny{43}};
\node[draw,circle,fill=black!9.5!white,inner sep=0,minimum size=4mm] () at (0.75,-4.875) {\tiny{39}};
\node[draw,circle,fill=black!6.25!white,inner sep=0,minimum size=4mm] () at (-0.75,-4.5) {\tiny{26}};
\node[draw,circle,fill=black!17.0!white,inner sep=0,minimum size=4mm] () at (-1.125,-4.5) {\tiny{69}};
\node[draw,circle,fill=black!11.75!white,inner sep=0,minimum size=4mm] () at (-0.75,-4.125) {\tiny{48}};
\node[draw,circle,fill=black!10.75!white,inner sep=0,minimum size=4mm] () at (-0.75,-4.875) {\tiny{44}};
\node[draw,circle,fill=black!4.5!white,inner sep=0,minimum size=4mm] () at (0.0,-5.25) {\tiny{19}};
\node[draw,circle,fill=black!12.0!white,inner sep=0,minimum size=4mm] () at (0.375,-5.25) {\tiny{49}};
\node[draw,circle,fill=black!19.5!white,inner sep=0,minimum size=4mm] () at (-0.375,-5.25) {\tiny{79}};
\node[draw,circle,fill=black!11.5!white,inner sep=0,minimum size=4mm] () at (0.0,-5.625) {\tiny{47}};
